FETA: Fairness Enforced Verifying, Training, and Predicting Algorithms for Neural Networks

Algorithmic decision making driven by neural networks has become very prominent in applications that directly affect people's quality of life. In this paper, we study the problem of verifying, training, and guaranteeing individual fairness of neural network models. A popular approach for enforcing fairness is to translate a fairness notion into constraints over the parameters of the model. However, such a translation does not always guarantee fair predictions of the trained neural network model. To address this challenge, we develop a counterexample-guided post-processing technique to provably enforce fairness constraints at prediction time. Contrary to prior work that enforces fairness only on points around test or train data, we are able to enforce and guarantee fairness on all points in the input domain. Additionally, we propose an in-processing technique to use fairness as an inductive bias by iteratively incorporating fairness counterexamples in the learning process. We have implemented these techniques in a tool called FETA. Empirical evaluation on real-world datasets indicates that FETA is not only able to guarantee fairness on-the-fly at prediction time but also is able to train accurate models exhibiting a much higher degree of individual fairness.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/evaluation.tex <==
%\golnoosh{add research questions}


In this section, we show the effectiveness of our proposed methods by performing empirical evaluations. For all the empirical evaluations that are presented in this section, we use three widely known real-world datasets:

\begin{itemize}
    \item German \cite{credit_bache2013uci}: This consists of 1000 samples with input dimension 61 and 3 sensitive attributes: sex \slash marital status (4 categories), age ($\in [19, 75])$, and foreign worker (2 categories). It is used for binary classification of good or bad credit risks.
    \item Adult \cite{adult_dataset}: This consists of 30k samples with input dimension 104 where there are four sensitive features: marital status (7 categories), race (5 categories), sex (2 categories), and native country (41 categories). The main task is to classify whether an individual's income exceeds \$50K per year.
\end{itemize}

All experiments were run on a machine with 10 GiB RAM and a 2.1GHz Intel Xeon processor. The implementations are all single-threaded. We use Gurobi-9.5.1\footnote{\url{https://www.gurobi.com}} as our solver.
% Our MIP models were solved using Gurobi-9.1.2\footnote{\url{https://www.gurobi.com}}.
The architecture used for the ReLU Neural Network is 3 hidden layers of size 16. It is trained via a 5-fold cross-validation with grid search over learning rate and batch size and early stopping to find the best model.

We first define a couple of metrics that facilitate addressing the research questions: i) \emph{CE Rate}: for how many test samples there exists an individual fairness counterexample, i.e., it is possible to change the outcome of the model by only changing the sensitive attributes, and ii) \emph{Flip Rate}: for how many test samples the prediction of the model should be flipped in order to guarantee individual fairness, i.e., not only a counterexample exists for them, but also the label of the counterexample is the majority vote. 

While these metrics only indicate the frequency of the fairness notion being violated, the average and maximum violation metrics indicate how severely the counterexamples violate the fairness notion, i.e., they are a surrogate for the frequency-based metrics.


\golnoosh{we should change the names! the name of the methods are not intuitive. Here is my suggestion:
\begin{itemize}
    \item Unfair baseline to NNs
    \item fair baseline to Fair-CE prediction
    \item retrained to Fair-CE training
    \item Fair retrained with FETA which is Fair-CE training and prediction 
    \item fair dummy should be the first row and it should be called the majority baseline
    \item we also need a blind model (model without sensitive features as an input)
\end{itemize}
}
\begin{table}[t]

    \begin{subtable}[t]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{|l||c|c|c|c|c|}
        \toprule
        \textbf{Model} &  \textbf{Accuracy (\%)} & \textbf{CE Rate (\%)} & \textbf{CE Count} & \textbf{Flip Rate (\%)} & \textbf{Inference Time (s)}\\
        \midrule
        Majority Baseline & $70.00 \pm 1.78$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.0 \pm 0.0$\\
        \midrule
        Blind Baseline & $75.70 \pm 3.17$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $\approx 0.0 \pm 0.0$\\
        \midrule
        Pretrained NN & $75.30 \pm 2.76$ & $33.10 \pm 9.36$ & $45.83 \pm 11.98$ & $7.30 \pm 2.54$ & $\approx 0.0 \pm 0.0$ \\
        \midrule
        Fair-CE Prediction & $74.80 \pm 4.14$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.52 \pm 0.11$\\
        \midrule
        Fair-CE Training & $75.90 \pm 0.66$ & $19.70 \pm 5.36$ & $28.93 \pm 4.27$ & $4.20 \pm 0.60$ & $\approx 0.0 \pm 0.0$  \\
        \midrule
        Fair-CE Train. and Pred. & $75.10 \pm 0.80$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.52 \pm 0.13$\\
        \bottomrule
        \end{tabular}}
        \caption{Summary of the results on the complete test set of German (full batch)}
    \end{subtable}
  
    \begin{subtable}[t]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{|l||c|c|c|c|c|}
        \toprule
        \textbf{Model} &  \textbf{Accuracy (\%)} & \textbf{CE Rate (\%)} & \textbf{CE Count} & \textbf{Flip Rate (\%)} & \textbf{Inference Time (s)}\\
        \midrule
        Majority Baseline & $74.29 \pm 0.88$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.0 \pm 0.0$\\
        \midrule
        Blind Baseline & $83.31 \pm 0.84$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $\approx 0.0 \pm 0.0$\\
        \midrule
        Pretrained NN & $84.11 \pm 1.04$ & $ \pm $ & $ \pm $ & $ \pm $ & $\approx 0.0 \pm 0.0$ \\
        \midrule
        Fair-CE Prediction & $ \pm $  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $ \pm $\\
        \midrule
        Fair-CE Training & $\pm $ & $ \pm $ & $\pm $ & $\pm$ & $\approx 0.0 \pm 0.0$  \\
        \midrule
        Fair-CE Train. and Pred. & $ \pm $ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $ \pm $\\
        \bottomrule
        \end{tabular}}
        \caption{Summary of the results on the Adult test set (ratio of $10\%$)}
        \label{tab:adult}
    \end{subtable}
    
    
    \begin{subtable}[t]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{|l||c|c|c|c|c|}
        \toprule
        \textbf{Model} &  \textbf{Accuracy (\%)} & \textbf{CE Rate (\%)} & \textbf{CE Count} & \textbf{Flip Rate (\%)} & \textbf{Inference Time (s)}\\
        \midrule
        Majority Baseline & $\pm$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.0 \pm 0.0$\\
        \midrule
        Blind Baseline & $80.11 \pm 1.44$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $\approx 0.0 \pm 0.0$\\
        \midrule
        Pretrained NN & $80.17 \pm 1.35$ & $ \pm $ & $ \pm $ & $ \pm $ & $\approx 0.0 \pm 0.0$ \\
        \midrule
        Fair-CE Prediction & $ \pm $  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $ \pm $\\
        \midrule
        Fair-CE Training & $\pm $ & $ \pm $ & $\pm $ & $\pm$ & $\approx 0.0 \pm 0.0$  \\
        \midrule
        Fair-CE Train. and Pred. & $ \pm $ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $ \pm $\\
        \bottomrule
        \end{tabular}}
        \caption{Summary of the results on the LawSchool test set (we train on a ratio of $2\%$ of the train set and test on a ratio of $10\%$ of the test set).}
        \label{tab:adult}
    \end{subtable}
    \caption{Summary of the results. \emph{CE Count} represents the average number of counterexamples per sample. \emph{Inference Time} corresponds to the average per-sample inference time. We use the counter-example guided counting to provide the guaranteed fair versions of the baseline and retrained models.}
\end{table}

\subsection{Empirical Results of Guaranteed Fair Predictions}
First, we will evaluate the guaranteed fair predictions algorithm by answering the following research questions:

\noindent\textbf{Q1: To what extent does our initial learned model violate individual fairness at prediction?}

The first row of Table \ref{tab:german} quantifies the amount of \emph{unfairness} in the initial model trained purely to increase performance. We observe a high amount of CE Rate, as well as CE Count. These two metrics explore the amount of unfairness in the whole input space. Moreover, Flip Rate indicates that a non-negligible portion of individuals in the test set are facing an unfair outcome.

While the mentioned metrics only indicate the frequency of fairness notion being disregarded, the average and maximum violations of the 0-th epoch in Figure \ref{fig:german} and \ref{fig:adult} indicate how severe unfairness is in the initial pre-trained model. Moreover, all fairness metrics drop to zero as we have guaranteed fairness in this case.

\noindent\textbf{Q2: What is the effect of guaranteed fair predictions on performance?}

As the first two rows in Table \ref{tab:german} indicate, we would not lose accuracy substantially, however, the extra per-sample run-time incurred at inference is high when we want to guarantee fairness.

\noindent\textbf{Q3: How scalable is our guaranteed fair predictions approach?}



\subsection{Empirical Results of Fairness Training}

We will now present an empirical evaluation of fairness-enforced learning. For this purpose, we address the following research questions:

\noindent\textbf{Q4: What is the effect of fairness-enforced retraining?}

Figure \ref{fig:german} and \ref{fig:adult} summarize the trajectory of fairness-enforced retraining over 50 epochs. Note that the initial model (epoch 0) is the baseline model pre-trained purely to maximize performance. We observe that while accuracy and loss oscillate toward fairness-performance tradeoff, violation curves and the number of counterexamples are going down. The substantial decrease in average and maximum violations indicates that the unfairness in the remaining counterexamples after retraining is much less severe. \kiarash{I think we should consider removing the Num of CE curve. Because it oscillates too much (unlike the violations curve) and we repeat it in the tables!}

\golnoosh{I agree, we don't need to show the number of CEs, thee max violation and AVG violation make more sense. And even to save space, we can select one of them} 
We minimize the $\ell_2$ distance to the Nadir point in order to choose a fairness-accuracy Pareto over the validation set. The Nadir point is the point with 100\% accuracy and 0 counterexamples. The third row in Table \ref{tab:german} indicates the performance of this model on the complete test set. We observe that while accuracy experiences another drop, CE Rate, CE Count, and Flip Rate are much less compared to the unfair baseline; at the same time, they provide similar inference time.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/german_batch_full.png}
    \caption{Learning curves for fairness-enforced re-training on the whole German dataset (ratio of $100\%$). Each row corresponds to a single metric and each column corresponds to a set of data on which the metrics are collected. Each curve is the mean over 5 folds and the shaded area represents the std.}
    \label{fig:german}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/adult.png}
%     \caption{Learning curves for fairness-enforced re-training on the Adult dataset (ratio of $10\%$). Each row corresponds to a single metric and each column corresponds to a set of data on which the metrics are collected. Each curve is the mean over 5 folds and the shaded area represents the std.}
%     \label{fig:adult}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/lawschool.png}
%     \caption{Learning curves for fairness-enforced re-training on the LawSchool dataset (ratio of $2\%$). Each row corresponds to a single metric and each column corresponds to a set of data on which the metrics are collected. Each curve is the mean over 5 folds and the shaded area represents the std.}
%     \label{fig:lawschool}
% \end{figure}

\noindent\textbf{Q5: ?}


\subsection{Empirical Results of \emph{FETA}}

Finally, we may leverage the verifiably fair predictions over the retrained model as well. These results are addressed in the following question:

\noindent\textbf{Q6: What is the effect of verification-guided fair prediction on the performance of the retrained model?}
 
The last row of Table \ref{tab:german} summarizes these results. We can observe that the drop in accuracy is less substantial as the model is already relatively fair. The fairness metrics are all 0 as the predictions are verifiably fair. Finally, we are still paying price in terms of runtime to obtain guaranteed fairness.

\noindent\textbf{Q7: ?}


==> table/ce-fair-training.tex <==
\begin{table}[h]
\centering
\caption{\aish{todo caption, check the results if they are correct}}
\resizebox{\linewidth}{!}{\footnotesize{
\begin{tabular}{l|lll|lll|lll}
\toprule
\textbf{Dataset} & \multicolumn{3}{c|}{German} & \multicolumn{3}{c}{IPUMS Adult } & \multicolumn{3}{c}{Law School}                                                                     \\ \midrule
                 & \multicolumn{1}{c}{\textbf{Accuracy}} & \multicolumn{1}{c}{\textbf{Flip Rate}} & \multicolumn{1}{c|}{\textbf{CE Rate}} & \multicolumn{1}{c}{\textbf{Accuracy}} & \multicolumn{1}{c}{\textbf{Flip Rate}} & \multicolumn{1}{c}{\textbf{CE Rate}} \\ \hline
\textbf{NN\textsubscript{b}}  & \\
\textbf{CE-Fair Prediction} & \\ 
\textbf{CE-Fair Training} & \\ 
\textbf{CE-Fair Train.+Predict.} & \\ 
\bottomrule
\end{tabular}}}
\label{tab:ce-fair-training}
\end{table}

==> table/results.tex <==

\begin{table}[h]
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{|l||c|c|c|c|}
        \toprule
        \textbf{Model} &  \textbf{Accuracy (\%)} & \textbf{Flip Rate (\%)} & \textbf{CE Rate (\%)} & \textbf{Inference Time (s)}\\
        \midrule
        \multicolumn{5}{|c|}{German}\\
        \midrule
        Majority Baseline & $70.00 \pm 1.78$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $\approx 0.0 \pm 0.0$\\
        \midrule
        Blind model & $70.30 \pm 2.20$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $3.8 \times 10^{-4} \pm 3.7 \times 10^{-4}$\\
        \midrule
        Pretrained NN (\textbf{NN\textsubscript{b}}) & $76.70 \pm 2.78$ & $8.90 \pm 0.73$ & $29.80 \pm 2.15$ & $1.9 \times 10^{-4} \pm 4.7 \times 10^{-5}$ \\
        \midrule
        CE-Fair Prediction & $74.20 \pm 3.50$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.45 \pm 0.06$\\
        \midrule
        CE-Fair Training & $75.70 \pm 3.77$ & $3.40 \pm .73$ & $17.70 \pm 4.67$ & $1.6 \times 10^{-4} \pm 4.4 \times 10^{-5}$  \\
        \midrule
        CE-Fair Train. and Pred. & $75.30 \pm 3.65$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.39 \pm 0.03$\\
        \midrule
        \multicolumn{5}{|c|}{IPUMS Adult}\\
        \midrule
        Majority Baseline & $54.61 \pm 0.55$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $\approx 0.0 \pm 0.0$\\
        \midrule
        Blind Model & $78.90 \pm 0.15$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $2.6 \times 10^{-4} \pm 6.5 \times 10^{-5}$\\
        \midrule
        Pretrained NN (\textbf{NN\textsubscript{b}}) & $81.57 \pm 0.47$ & $24.39 \pm 1.52$ & $89.40 \pm 1.80$ & $2.5 \times 10^{-3} \pm 1.5 \times 10^{-3}$ \\
        \midrule
        CE-Fair Prediction & $73.23 \pm 0.93$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $119.64 \pm 33.45$\\
        \midrule
        CE-Fair Training & $80.03 \pm 0.57$ & $2.80 \pm 0.67$ & $15.34 \pm 2.53$ & $5.7 \times 10^{-4} \pm 1.9 \times 10^{-4}$  \\
        \midrule
        CE-Fair Train. and Pred. & $79.46 \pm 0.71$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $10.20 \pm 2.90$\\
        \midrule
        \multicolumn{5}{|c|}{Law School}\\
        \midrule
        Majority Baseline & $72.98 \pm 0.50$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $\approx 0.0 \pm 0.0$\\
        \midrule
        Blind model & $74.19 \pm 1.20$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $2.6 \times 10^{-4} \pm 4.5 \times 10^{-5}$\\
        \midrule
        Pretrained NN (\textbf{NN\textsubscript{b}}) & $82.72 \pm 0.19$ & $17.53 \pm 0.59$ & $41.18 \pm 2.05$ & $2.5 \times 10^{-4} \pm 9.4 \times 10^{-6}$ \\
        \midrule
        CE-Fair Prediction & $74.36 \pm 1.95$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.39 \pm 0.14$\\
        \midrule
        CE-Fair Training & $84.99 \pm 0.28$ & $5.06 \pm 0.97$ & $7.64 \pm 0.89$ & $1.4 \times 10^{-4} \pm 2.4 \times 10^{-5}$  \\
        \midrule
        CE-Fair Train. and Pred. & $84.14 \pm 0.97$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.30 \pm 0.13 $\\
        \bottomrule
        \end{tabular}}
    \caption{Summary of the results. We use the CE-Fair Predictions to provide the guaranteed fair versions of the pretrained and retrained NN models.}
    \label{tab:all}
\end{table}


% \begin{table}[t]{\linewidth}
%         \centering
%         \resizebox{\linewidth}{!}{\footnotesize{
%         \begin{tabular}{|l||c|c|c|c|c|}
%         \toprule
%         \textbf{Model} &  \textbf{Accuracy (\%)} & \textbf{Flip Rate (\%)} & \textbf{CE Rate (\%)} & \textbf{CE Count} & \textbf{Inference Time (s)}\\
%         \midrule
%         \multicolumn{6}{|c|}{German ($\rho = 100\%$)}\\
%         \midrule
%         Majority Baseline & $70.00 \pm 1.78$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $\approx 0.0 \pm 0.0$\\
%         \midrule
%         Blind model & $74.40 \pm 3.61$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $2.2 \times 10^{-4} \pm 6.5 \times 10^{-5}$\\
%         \midrule
%         Pretrained NN & $76.70 \pm 2.78$ & $8.90 \pm 0.73$ & $29.80 \pm 2.15$ & $42.89 \pm 1.62$ & $1.9 \times 10^{-4} \pm 4.7 \times 10^{-5}$ \\
%         \midrule
%         CE-Fair Prediction & $74.20 \pm 3.50$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.45 \pm 0.06$\\
%         \midrule
%         CE-Fair Training & $75.70 \pm 3.77$ & $3.40 \pm .73$ & $17.70 \pm 4.67$ & $24.57 \pm 6.52$ & $1.6 \times 10^{-4} \pm 4.4 \times 10^{-5}$  \\
%         \midrule
%         CE-Fair Train. and Pred. & $75.30 \pm 3.65$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.39 \pm 0.03$\\
%         \midrule
%         \multicolumn{6}{|c|}{Adult ($\rho = 10\%$)}\\
%         \midrule
%         Majority Baseline & $74.29 \pm 0.88$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $\approx 0.0 \pm 0.0$\\
%         \midrule
%         Blind model & $83.74 \pm 0.80$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $1.7 \times 10^{-4} \pm 1.7 \times 10^{-5}$\\
%         \midrule
%         Pretrained NN & $83.98 \pm 1.23$ & $8.98 \pm 2.07$ & $50.18 \pm 12.76$ & $17535 \pm 4104.63$ & $2.6 \times 10^{-4} \pm 1.1 \times 10^{-5}$ \\
%         \midrule
%         CE-Fair Prediction & $81.89 \pm 1.45$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $15.34 \pm 3.36$\\
%         \midrule
%         CE-Fair Training & $83.05 \pm 1.34$ & $6.89 \pm 3.30$ & $27.89 \pm 15.47$ & $10847.9 \pm 5750.17$ & $2.4 \times 10^{-4} \pm 1.0 \times 10^{-5}$  \\
%         \midrule
%         CE-Fair Train. and Pred. & $81.19 \pm 1.49$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $12.54 \pm 5.79$\\
%         \midrule
%         \multicolumn{6}{|c|}{IPUMS Adult ($\rho = 1\%$)}\\
%         \midrule
%         Majority Baseline & $54.94 \pm 5.60$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $\approx 0.0 \pm 0.0$\\
%         \midrule
%         Blind model & $76.92 \pm 1.96$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $2.4 \times 10^{-4} \pm 2.2 \times 10^{-5}$\\
%         \midrule
%         Pretrained NN & $79.12 \pm 5.93$ & $28.79 \pm 6.19$ & $91.86 \pm 2.03$ & $53440.1 \pm 2839.51$ & $5.4 \times 10^{-4} \pm 7.7 \times 10^{-5}$ \\
%         \midrule
%         CE-Fair Prediction & $71.42 \pm 5.24$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $127.63 \pm 30.62$\\
%         \midrule
%         CE-Fair Training & $78.68 \pm 3.23$ & $3.07 \pm 2.13$ & $16.26 \pm 6.03$ & $5632.3 \pm 3650.59$ & $2.7 \times 10^{-4} \pm 2.2 \times 10^{-5}$  \\
%         \midrule
%         CE-Fair Train. and Pred. & $79.12 \pm 2.86$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $9.15 \pm 5.7$\\
%         \midrule
%         \multicolumn{6}{|c|}{Law School ($\rho = 100\%$)}\\
%         \midrule
%         Majority Baseline & $72.98 \pm 0.50$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $\approx 0.0 \pm 0.0$\\
%         \midrule
%         Blind model & $82.13 \pm 0.62$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $2.4 \times 10^{-4} \pm 1.8 \times 10^{-5}$\\
%         \midrule
%         Pretrained NN & $82.72 \pm 0.19$ & $17.53 \pm 0.59$ & $41.18 \pm 2.05$ & $1.19 \pm 0.04$ & $2.5 \times 10^{-4} \pm 9.4 \times 10^{-6}$ \\
%         \midrule
%         CE-Fair Prediction & $74.36 \pm 1.95$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.39 \pm 0.14$\\
%         \midrule
%         CE-Fair Training & $84.99 \pm 0.28$ & $5.06 \pm 0.97$ & $7.64 \pm 0.89$ & $0.25 \pm 0.03$ & $1.4 \times 10^{-4} \pm 2.4 \times 10^{-5}$  \\
%         \midrule
%         CE-Fair Train. and Pred. & $84.14 \pm 0.97$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.30 \pm 0.13 $\\
%         \bottomrule
%         \end{tabular}}}
%     \caption{Summary of the results. \emph{CE Count} represents the average number of counterexamples per sample. \emph{Inference Time} corresponds to average per-sample inference time. We use the counter-example guided counting to provide the guaranteed fair versions of the baseline and retrained models.}
%     \label{tab:all}
% \end{table}



% \begin{table}[t]{\linewidth}
%         \centering
%         \resizebox{\linewidth}{!}{\footnotesize{
%         \begin{tabular}{|l||c|c|c|c|c|}
%         \toprule
%         \textbf{Model} &  \textbf{Accuracy (\%)} & \textbf{Flip Rate (\%)} & \textbf{CE Rate (\%)} & \textbf{CE Count} & \textbf{Inference Time (s)}\\
%         \midrule
%         \multicolumn{6}{|c|}{German ($\rho = 100\%$)}\\
%         \midrule
%         Majority Baseline & $70.00 \pm 1.78$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $\approx 0.0 \pm 0.0$\\
%         \midrule
%         Blind model & $74.40 \pm 3.61$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $2.2 \times 10^{-4} \pm 6.5 \times 10^{-5}$\\
%         \midrule
%         Pretrained NN & $76.70 \pm 2.78$ & $8.90 \pm 0.73$ & $29.80 \pm 2.15$ & $42.89 \pm 1.62$ & $1.9 \times 10^{-4} \pm 4.7 \times 10^{-5}$ \\
%         \midrule
%         CE-Fair Prediction & $74.20 \pm 3.50$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.45 \pm 0.06$\\
%         \midrule
%         CE-Fair Training & $76.10 \pm 2.81$ & $3.50 \pm 1.51$ & $17.60 \pm 5.88$ & $24.56 \pm 6.94$ & $1.6 \times 10^{-4} \pm 4.4 \times 10^{-5}$  \\
%         \midrule
%         CE-Fair Train. and Pred. & $75.20 \pm 2.94$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.39 \pm 0.03$\\
%         \midrule
%         \multicolumn{6}{|c|}{IPUMS Adult ($\rho = 1\%$)}\\
%         \midrule
%         Majority Baseline & $54.94 \pm 5.60$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $\approx 0.0 \pm 0.0$\\
%         \midrule
%         Blind model & $76.92 \pm 1.96$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $2.4 \times 10^{-4} \pm 2.2 \times 10^{-5}$\\
%         \midrule
%         Pretrained NN & $79.12 \pm 5.93$ & $28.79 \pm 6.19$ & $91.86 \pm 2.03$ & $53440.1 \pm 2839.51$ & $5.4 \times 10^{-4} \pm 7.7 \times 10^{-5}$ \\
%         \midrule
%         CE-Fair Prediction & $71.42 \pm 5.24$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $127.63 \pm 30.62$\\
%         \midrule
%         CE-Fair Training & $81.67 \pm 0.26$ & $3.07 \pm 2.13$ & $16.26 \pm 6.03$ & $5632.3 \pm 3650.59$ & $2.7 \times 10^{-4} \pm 2.2 \times 10^{-5}$  \\
%         \midrule
%         CE-Fair Train. and Pred. & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $9.15 \pm 5.7$\\
%         \midrule
%         \multicolumn{6}{|c|}{Law School ($\rho = 100\%$)}\\
%         \midrule
%         Majority Baseline & $72.98 \pm 0.50$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $\approx 0.0 \pm 0.0$\\
%         \midrule
%         Blind model & $82.13 \pm 0.62$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $2.4 \times 10^{-4} \pm 1.8 \times 10^{-5}$\\
%         \midrule
%         Pretrained NN & $82.72 \pm 0.19$ & $17.53 \pm 0.59$ & $41.18 \pm 2.05$ & $1.19 \pm 0.04$ & $2.5 \times 10^{-4} \pm 9.4 \times 10^{-6}$ \\
%         \midrule
%         CE-Fair Prediction & $74.36 \pm 1.95$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.39 \pm 0.14$\\
%         \midrule
%         CE-Fair Training & $83.74 \pm 1.26$ & $4.23 \pm 1.86$ & $7.36 \pm 2.30$ & $0.22 \pm 0.08$ & $1.4 \times 10^{-4} \pm 2.4 \times 10^{-5}$  \\
%         \midrule
%         CE-Fair Train. and Pred. & $82.58 \pm 1.21$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.30 \pm 0.13 $\\
%         \bottomrule
%         \end{tabular}}}
%     \caption{New results}
%     \label{tab:all3}
% \end{table}
